Improving Differential-Neural Distinguisher Model For DES, Chaskey, and PRESENT

In CRYPTO'19, Gohr proposed a new cryptanalysis strategy using machine learning algorithms. Combining the differential-neural distinguisher with a differential path and integrating the advanced key recovery procedure, Gohr achieved a 12-round key recovery attack on Speck32/64. Chen and Yu improved prediction accuracy of differential-neural distinguisher considering derived features from multiple-ciphertext pairs instead of single-ciphertext pairs. By modifying the kernel size of initial convolutional layer to capture more dimensional information, the prediction accuracy of differential-neural distinguisher can be improved for for three reduced symmetric ciphers. For DES, we improve the prediction accuracy of (5-6)-round differential-neural distinguisher and train a new 7-round differential-neural distinguisher. For Chaskey, we improve the prediction accuracy of (3-4)-round differential-neural distinguisher. For PRESENT, we improve the prediction accuracy of (6-7)-round differential-neural distinguisher. The source codes are available in https://drive.google.com/drive/folders/1i0RciZlGZsEpCyW-wQAy7zzJeOLJNWqL?usp=sharing.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother


==> tex/02-00-Preliminary.tex <==
\section{Preliminary}

